Mean Value Theorems for Riemannian Manifolds via the Obstacle Problem

We develop some of the basic theory for the obstacle problem on Riemannian Manifolds, and we use it to establish a mean value theorem. Our mean value theorem works for a very wide class of Riemannian manifolds and has no weights at all within the integral.

==> macros.tex <==
\newcommand{\nc}[2]{ \newcommand{#1}{#2} }
\newcommand{\pnu}[1]{ \ensuremath{\frac{\partial #1}{\partial\nu}} }
% partial derivative in the normal direction
\nc{\avint}{ {- \hspace{-3.5mm} \int} }  % average integral
\newcommand{\myavint}[1]{ \int_{#1} \mkern-27mu
                          \rule[.033 in]{.12 in}{.01 in} \ \ \  }
\nc{\R}{\rm I \! R}  % Real Numbers
\nc{\N}{\rm I \! N}  % Natural Numbers
\newcommand{\closure}[1]{ \stackrel{\rule{.1 in}{.01 in}}{#1} }
\newcommand{\dclosure}[1]{ \stackrel{\rule{.2 in}{.01 in}}{#1} }
\newcommand{\tclosure}[1]{ \stackrel{\rule{.3 in}{.01 in}}{#1} }
\newcommand{\qclosure}[1]{ \stackrel{\rule{.4 in}{.01 in}}{#1} }
\newcommand{\norm}[4]{ || #1 ||_{_{{ #2 }^{ #3 }( #4 )}} }
\newcommand{\chisub}[1]{ {\mathbf{\chi}}_{_{#1}} }

\newcommand{\newsec}[2]{ \section{#1} \label{sec-#2}  % starts new section,
                         \setcounter{equation}{0}     % resets counters,
                         \setcounter{theorem}{0} }    % makes label
\newcommand{\newsub}[2]{ \subsection{#1} \label{sub-#2} }
% starts new subsection, makes label
\newcommand{\refeqn}[1]{ (\!\!~\ref{eq:#1}) } % gives references to
\newcommand{\refthm}[1]{ (\!\!~\ref{#1}) }    % equations or theorems

\nc{\Holder}{H\"{o}lder\ }
\newcommand{\vhat}[1]{ \hat{\mathbf{#1}} }
\newcommand{\vnorm}[1]{ ||\vec{#1}|| }
\newcommand{\parder}[2]{ \frac{\partial #1}{\partial #2} }
\newcommand{\dotvecs}[2]{ \vec{#1} \bullet \vec{#2} }
\newcommand{\crvecs}[2]{ \vec{#1} \times \vec{#2} }
\nc{\ith}{ \ensuremath{\text{i}^{\text{th}}} }
\nc{\jth}{ \ensuremath{\text{j}^{\text{th}}} }
\nc{\kth}{ \ensuremath{\text{k}^{\text{th}}} }
\nc{\dst}{ \ensuremath{\text{1}^{\text{st}}_{\delta}} }
\nc{\dnd}{ \ensuremath{\text{2}^{\text{nd}}_{\delta}} }
\nc{\ost}{ \ensuremath{\text{1}^{\text{st}}} }
\nc{\tnd}{ \ensuremath{\text{2}^{\text{nd}}} }
\nc{\curl}{ \nabla \times }
\nc{\Div}{ \nabla \cdot }
\nc{\DC}{K}

\newcommand{\BVP}[4]{  % 1 = equation, 2 = bdry vals, 3 = label, 4 = set.
  \begin{equation}
        \begin{array}{rl}
           #1 & \ \text{in}
               \ \ #4 \vspace{.05in} \\
           #2 & \ \text{on} \ \ \partial #4 \;.
        \end{array}
  \label{eq:#3}
  \end{equation}    }
\newcommand{\BVPom}[3]{   \BVP{#1}{#2}{#3}{ \Omega }  }
\newcommand{\BVPb}[3]{   \BVP{#1}{#2}{#3}{ B_{1} }  }
\newcommand{\BVPc}[4]{  % 1 = equation, 2 = bdry vals, 3 = label, 4 = set.  (The extra ``c'' stands for ``comma'')
  \begin{equation}
        \begin{array}{rl}
           #1 & \ \text{in}
               \ \ #4 \vspace{.05in} \\
           #2 & \ \text{on} \ \ \partial #4 \;,
        \end{array}
  \label{eq:#3}
  \end{equation}    }
\newcommand{\BVPcom}[3]{   \BVP{#1}{#2}{#3}{ \Omega }  }
\newcommand{\BVPcb}[3]{   \BVP{#1}{#2}{#3}{ B_{1} }  }

\nc{\Ppl}{ \mathcal{M}^{+} }  \nc{\Pmn}{ \mathcal{M}^{-} }

\nc{\smiley}{ $\stackrel{\because}{\smile} \;$ }



